Coexistence Gaps in Space: Cross-Technology Interference-Nulling for Improving LTE-U/WiFi Coexistence

To avoid the foreseeable spectrum crunch, LTE operators have started to explore the option to directly use 5 GHz unlicensed spectrum band being used by IEEE 802.11 (WiFi). However, as LTE is not designed with shared spectrum access in mind, there is a major issue of coexistence with WiFi networks. Current coexistence schemes to be deployed at the LTE-U BS create coexistence gaps only in one domain (e.g., time, frequency, or space) and can provide only incremental gains due to the lack of coordination among the coexisting WiFi and LTE-U networks. Therefore, we propose a coordinated coexistence scheme which relies on cooperation between neighboring LTE-U and WiFi networks. Our proposal suggests that LTE-U BSs equipped with multiple antennas can create coexistence gaps in space domain in addition to the time domain gaps by means of cross-technology interference nulling towards WiFi nodes in the interference range. In return, LTE-U can increase its own airtime utilization while trading off slightly its antenna diversity. The cooperation offers benefits to both LTE-U and WiFi in terms of improved throughput and decreased channel access delay. More specifically, system-level simulations reveal a throughput gain up to 221% for LTE-U network and 44% for WiFi network depending on the setting, e.g., the distance between the two cell, number of LTE antennas, and WiFi users in the LTE-U BS neighborhood. Our proposal provides significant benefits especially for moderate separation distances between LTE-U/WiFi cells where interference from a neighboring network might be severe due to the hidden network problem.

==> abs.tex <==
%!TEX root = main_template.tex
\begin{abstract}

To avoid the foreseeable spectrum crunch, LTE operators have started to explore the option to directly use 5\,GHz unlicensed spectrum band being used by IEEE 802.11~(WiFi).
%
However, as LTE is not designed with shared spectrum access in mind, there is a major issue of coexistence with WiFi networks.
% DONE: \tolja{I would remove the second part: } which implement listen-before-talk medium access and therefore lose the channel to LTE unlicensed (LTE-U).
%
Current coexistence schemes to be deployed at the LTE-U BS create coexistence gaps only in one domain~(e.g., time, frequency, or space) and can provide only incremental gains due to the lack of coordination among the coexisting WiFi and LTE-U networks.
% to improve the coexistence-friendliness of the LTE-U introduce coexistence gaps in either frequency, time, or space domain to leave the medium fairly to WiFi.
%
% Although mitigating the resulting mutual interference of WiFi and LTE-U on each other,
% However, the achieved gains are limited due to the uncoordinated operation of such coexistence schemes.
%
Therefore, we propose a coordinated coexistence scheme which relies on cooperation between neighboring LTE-U and WiFi networks.
%
Our proposal suggests that LTE-U BSs equipped with multiple antennas can create coexistence gaps 
in space domain in addition to the time domain gaps by means of cross-technology interference nulling towards WiFi nodes in the interference range. In return, LTE-U can increase its own airtime utilization while trading off slightly its antenna diversity.
%
The cooperation offers benefits to both LTE-U and WiFi in terms of improved throughput and decreased channel access delay.
%
More specifically, system-level simulations reveal a throughput gain up to \maxLTEgainthru\% for LTE-U network and \maxWiFigainthru\% for WiFi network depending on the setting, e.g., distance between the two cell, number of LTE antennas, and WiFi users in the LTE-U BS neighborhood.
%\tolja{I run a simulations with only a single WiFi client. Here the gain for WiFi larger: . Maybe it would good to show.}
%
%In line with the literature, 
Our proposal provides significant benefits especially for moderate separation distances between LTE-U/WiFi cells where interference from a neighboring network might be severe due to the hidden network problem.
%\tolja{The abstract is too long for my taste. Moreover it contains lots of things normally being part of the introduction. I would suggest to shrink it by 50\%.}

% \su{Check if the discussions and above numbers are still valid for figures from the new simulations.}
% \su{WiFi does not get much throughput gain but it has a faster access to the channel. We need to quantify this using LTE-airtime and the LTE-on period. Discuss that although under interference we can decode the packets using error correction?.}



%\tolja{What is this paper about? This paper is just a theoretical analysis of the gain from cross-technology interference-nulling from LTE-U towards WiFi. We do not say how such a cross-technology interference-nulling can be implemented in a practical system. This is the objective of our other paper CTCbeam. Hence, I completely removed the description of LtFi in the primer. I only mentioned in the conclusions that LtFi might be an enabler for a practical solution. This is important as we in this paper do not say how the LTE-BS is getting the information needed to calculate the beam weights for the nulling. In our simulations we assumed that the LTE-BS has perfect channel state information (CSI) of its channel towards any WiFi node in proximity. We have to explicitly mention this - availability of perfect cross-tech CSI at LTE-U BS. Obtaining this information is a challenge for a practical system as our assumption is that WiFi is unable to decode LTE-U frames - which is needed to obtain CSI. In CTCbeam we do not need this. Instead we perform random interference-nulling and use the LtFi cross-tech control channel to steer the nulling beam in the proper direction. Our problem is that we cannot cite the CTCbeam as it is not yet ready. So we have to explain the practical considerations very carefully without mentioning the idea behind CTCbeam.}



%Basic idea: With LtFi we showed that it is possible to create a cross-technology control channel (CTC) between LTE-U and WiFi. In this paper we leverage that to perform interference management between these two heterogeneous technologies. We assume that a LTE-U BS is equipped with an antenna array (e.g. ULA). Co-existence is achieved by utilizing the degrees of freedom of LTE-U BS to perform nulling towards co-located WiFi nodes. The challenge is that complex channel state information (CSI) cannot be obtained from the CTC. Hence, we aim for an indirect approach using random nulling scheme and binary search. In each round/level the WiFi node feedbacks the null configuration with the lowest PER in the LTE-U on period to the LTE-BS whereas the seach continues with narrower null beam on the next level.

%\tolja{We analyze the tradeoff between interference nulling and CSAT duty cycle length. Basic idea: if LTE-U is nulling out its interference towards $N$ out of $P$ WiFi nodes it is able to increase its CSAT duty cycle from $\frac{1}{P+1}$ to $\frac{1}{P+1-N}$. However, at a loss in SNR towards its own UEs. Hence there must be a optimal number of nulls, right?}

%\tolaj{TBD}

\end{abstract}
